A Novel Two-Step Fine-Tuning Pipeline for Cold-Start Active Learning in Text Classification Tasks

This is the first work to investigate the effectiveness of BERT-based contextual embeddings in active learning (AL) tasks on cold-start scenarios, where traditional fine-tuning is infeasible due to the absence of labeled data. Our primary contribution is the proposal of a more robust fine-tuning pipeline - DoTCAL - that diminishes the reliance on labeled data in AL using two steps: (1) fully leveraging unlabeled data through domain adaptation of the embeddings via masked language modeling and (2) further adjusting model weights using labeled data selected by AL. Our evaluation contrasts BERT-based embeddings with other prevalent text representation paradigms, including Bag of Words (BoW), Latent Semantic Indexing (LSI), and FastText, at two critical stages of the AL process: instance selection and classification. Experiments conducted on eight ATC benchmarks with varying AL budgets (number of labeled instances) and number of instances (about 5,000 to 300,000) demonstrate DoTCAL's superior effectiveness, achieving up to a 33% improvement in Macro-F1 while reducing labeling efforts by half compared to the traditional one-step method. We also found that in several tasks, BoW and LSI (due to information aggregation) produce results superior (up to 59% ) to BERT, especially in low-budget scenarios and hard-to-classify tasks, which is quite surprising.

==> sections/intro.tex <==
\section{Introduction} \label{sec:intro}

Two of the most challenging issues of the supervised automatic text classification (ATC) task are: (i) how to represent textual data in meaningful, machine-tractable ways~\citep{Cunha_2021} and (ii) how to reduce the costs of obtaining labeled data to train classification models~\citep{Settles2010}.\looseness=-1

Regarding the first issue, contextual embeddings such as those produced by Bidirectional Encoder from Transformers or BERT~\citep{devlin2019bert} have produced state-of-the-art results  for a large (but not exhaustive) range of ATC tasks. These embeddings are pre-trained to capture general linguistic patterns from large external collections of unlabeled documents and can be adjusted to more specific domains by means of a fine-tuning process.\looseness=-1

Solutions to the second issue frequently involve active learning (AL) strategies, which aim to select, among the often abundant set of unlabeled data, only the most ``informative'' (diversified and representative) data instances to label.  An AL process can be divided into two stages, illustrated at the top of Figure 1: (i) the selection stage, which aims at selecting informative instances to label, and (ii) the classification stage, in which we train a classification model using the instances selected in stage (i), after being actively labeled. In each stage, textual data must be properly represented (e.g., with contextual embeddings), illustrated in Figure 1 as rounded rectangles. At the start of stage (i), no fine-tuning for ATC can be performed since there is still no labeled data, a scenario referred to as \textbf{cold-start}. Besides that, the number of instances selected in stage (i) is typically limited to a given \textit{budget} or the \textit{maximum number of instances} one can afford to label, as the cost and complexity of labeling data are non-negligible.\looseness=-1

In this context, we aim to tackle the ``cold-start'' active learning problem for ATC under the (text) representation perspective, that is, we aim to investigate how different representation approaches impact AL effectiveness considering different budget sizes. Despite the success of contextual embeddings for ATC, little has been investigated regarding their  effectiveness in the selection phase of the AL, \textit{especially in a cold-start scenario in which there is no labeled data available (and no fine-tuning is possible)}. One of the few studies that evaluate contextual embeddings for AL~\citep{emnlp_2020} only performs a direct fine-tuning process with already labeled data to adapt the produced embeddings to the target classification task. We refer to this traditional fine-tuning method as \textbf{one-step fine-tuning}, illustrated in Figure 1-b. In most AL settings, the labeled dataset is still under construction and is typically small (due to low budgets in the beginning of the process), which may be detrimental to the effectiveness of this traditional fine-tuning method.\looseness=-1

Thus, it is desirable  to invest in more robust fine-tuning processes for AL which reduce the need for labeled data. Accordingly, in this article, as our \textbf{first contribution} we propose to improve AL methods that exploit contextual embeddings by means of a novel \textbf{two-step} \textit{fine-tuning pipeline} named DoTCAL (\textbf{Do}main and \textbf{T}ask Adaptation for \textbf{C}old-Start \textbf{A}ctive \textbf{L}earning (Figure 1-a), consisting of two phases: (i) a domain-oriented adaptation of the model, exploiting all available unlabeled training data and (ii) a further adaptation of the model using the training samples that were actively labeled after being selected by the AL process (task adaptation). More specifically, while in step (i) we continue the model adaptation to the target domain by pretraining using a masked language modeling (MLM) objective (slot-filling with words), in step (ii), model weights are adjusted using the ATC objective function.  We hypothesize that this new  two-step process allows higher classification effectiveness with a lower labeling effort when compared to the direct, one-step fine-tuning, since our approach takes advantage of all the domain-specific available unlabeled data. To the best of our knowledge, no previous work has proposed nor evaluated such  two-step fine-tuning approach for AL.\looseness=-1

An important aspect to investigate in this novel two-step fine-tuning pipeline is which textual representation to exploit. In the selection stage of cold-start AL, we can choose among non-fine-tuned embeddings or domain-adapted embeddings (first step of our DoTCAL approach), since no labeled data is available. In the classification stage,  all options (rounded rectangles in Figure 1) are available, but the labeled set is usually small in the beginning of the process, especially with low budgets. It is not completely clear that the same contextual embedding representation that constitutes the state-of-the art for a fully labeled dataset is the best for AL, especially as input for the selection stage or for the classification stage.\looseness=-1

In this context, we compare contextual embeddings  with other popular text representation paradigms, such as bag-of-words (BoW) and Latent Semantic Indexing (LSI) for the selection as well as the classification phase, considering limited labeling budgets. BoW is still effective in many tasks~\citep{Cunha_2021} while LSI reduces the original term-document matrix to a lower dimensional space, minimizing information loss by exploiting ``more compressed'' latent terms shared by many instances~\citep{LSI}. This approach is suitable in an AL task in which we are interested in selecting only a few representative examples from the whole dataset to label.\looseness=-1

As our \textbf{second contribution}, we evaluate, under different budget scenarios, the effectiveness of these different text representation approaches in each AL stage (selection and classification). More specifically, we aim to answer the following research questions (RQs):\looseness=-1

\noindent \textit{RQ1: How much can we improve AL effectiveness using the proposed two-step fine-tuning (DoTCAL) pipeline?}\looseness=-1

\noindent \textit{RQ2: How does the chosen representation for text impact the selection of highly representative and diverse instances under different budgets?}\looseness=-1

\noindent \textit{RQ3: How does the chosen text representation given as input for the classifier impact classification effectiveness under different budgets?}\looseness=-1

Towards answering these questions, we exploit a state-of-the-art AL strategy in the cold-start scenario named Density Weighted Diversity Based Query Strategy (DWDS) \citep{wang_cswd2021}. This method tackles the selection of informative instances, which is a combinatorial optimization problem, by performing a greed (though extended by a beam-search mechanism) selection of instances with high density (highly representative), discarding those that are similar to other selected instances, also promoting diversity.\looseness=-1

We evaluate this approach using eight ATC datasets under different active labeling budgets. We also vary the representation exploited in each stage of the AL process.  Regarding RQ1, our results show that the 2-step fine-tuning process allows higher classification effectiveness, with gains of up to 33\% in macro-F1 in small budget scenarios and with a lower labeling effort compared to the direct, 1-step fine-tuning. Typically, to reach a given classification effectiveness, our DoTCAL pipeline requires half of the number of labeled instances needed by the traditional 1-step process.\looseness=-1

\begin{figure*}[t]
\hspace{-0.3cm}
    \centering
    \includegraphics[width=0.999\textwidth]{img/finetuning.png}
    \caption{Cold-Start Active Learning for ATC and contextual embeddings fine-tuning approaches}
    \label{fig:al}
\end{figure*}

Answering RQ2, despite some resilience to different representations in the selection stage, the best approach depends on the dataset. Generally, this best approach is the same representation  used in the classification stage: BoW/LSI for some datasets and BERT for others.\looseness=-1

Regarding RQ3, although contextual embeddings constitute a state-of-the-art representation for ATC (BERT wins in 5 out of 8 evaluated datasets, for all budget scenarios), BoW and LSI lead to the best classification results in other 3 hard-to-classify datasets. Comparing BoW and LSI, the latter outperforms the former for low-budget scenarios (under 200 labeled instances), confirming our hypothesis that latent dimensions are advantageous when training with  small sets of labeled instances since it aggregates information of many instances into fewer dimensions.\looseness=-1

After evaluating BERT-based contextual embeddings, which are one of the most popular, general-use and low cost (in terms of memory usage) contextual embeddings, we also provide results for a larger robust model, namely RoBERTa \citep{roberta}. Our experiments demonstrate the superiority of the DoTCAL fine-tuning process w.r.t the traditional 1-step fine-tuning, with gains of up to 27\% in Macro-F1, despite some advantage RoBERTa presents for low labeling budgets.

Summarizing, our main contributions are two-fold. First, we propose DoTCAL, a new two-step fine-tuning pipeline for contextual embeddings that outperforms previous one-step SOTA solutions regarding a tradeoff effectiveness-cost (budget size). Second we provide a thorough empirical study  showing the benefits of different text representations in different contexts (datasets) under different budgets in different stages of the AL process.\looseness=-1

\paragraph{Article Organization:} The rest of this paper is organized as follows. Section \ref{sec:related} presents related studies, while Section \ref{sec:statement} formally defines our addressed problem. Section \ref{sec:methodology} describes the evaluated representation and AL approaches, while Section \ref{sec:setup} describes the experimental setup. Section \ref{sec:results} presents our results, while Section \ref{sec:discussion} presents a discussion of the theoretical and practical implications of our study. Finally, Section \ref{sec:conc} provides conclusions and directions for future work.\looseness=-1
